Random Order Set Cover is as Easy as Offline

We give a polynomial-time algorithm for OnlineSetCover with a competitive ratio of $O(\log mn)$ when the elements are revealed in random order, essentially matching the best possible offline bound of $O(\log n)$ and circumventing the $\Omega(\log m \log n)$ lower bound known in adversarial order. We also extend the result to solving pure covering IPs when constraints arrive in random order. The algorithm is a multiplicative-weights-based round-and-solve approach we call LearnOrCover. We maintain a coarse fractional solution that is neither feasible nor monotone increasing, but can nevertheless be rounded online to achieve the claimed guarantee (in the random order model). This gives a new offline algorithm for SetCover that performs a single pass through the elements, which may be of independent interest.

==> polytime.tex <==

	\section{A Polynomial Time Algorithm for the Unit Cost Setting}
	
	\label{sec:poly}
	
	Unfortunately we cannot afford to maintain a list of all $O(m^k)$ possible $k$-tuples that cover the elements seen so far, since in general $k = \omega(1)$. 
	However, we can reuse the intuition that we either make progress in covering or make progress learning about the optimal solution.
	Instead of a collection of ``good'' $k$-tuples, we will
        maintain a distribution $x$ on sets, and update it via a
        multiplicative weights rule.
	
	\begin{algorithm}[H]
	\caption{\textsc{RandomOrderSetCover}}
	\label{alg:unitcost}
	\begin{algorithmic}[1]
		\State Initialize $x^{(1)}$ to the uniform distribution: for every $S$, set $x_S \leftarrow \frac{1}{m}$.
		\For{$t=1,2,\ldots$}		
		\State{$v \leftarrow$ $t$-th element in the
			random order.}
		\If {$v$ already covered}
		\State Do nothing.
		\Else
			\State Buy $S \sim x{(t)}$, a single random draw from $x$.
			\If {$x^{(t-1)}_v < 1$}
			\State Let $Z^{(t)} = \sum_{S \ni v} e\cdot
			x^{(t-1)}_S + \sum_{S \not \ni v} x^{(t-1)}_S$.
			\State For every set $S$, update $x^{(t)}_S \leftarrow
			x^{(t-1)}_S \cdot \exp\left\{\mathbbm{1}\{S \ni v\}\right\} /
			Z^{(t)}$.
			\EndIf
			\If{$v$ still uncovered}
			\State Buy arbitrary set covering $v$.
			\EndIf
		\EndIf
		\EndFor 
	\end{algorithmic}
\end{algorithm}
	
	Note the important detail that we only perform the multiplicative weight update when an element arrives and that element is uncovered by the sets bought so far.
	
		\begin{theorem}
	    \label{thm:unit_cost_poly}
		For the unit cost setting, there is a polynomial time randomized algorithm achieving competitive ratio $O(\log (mn/k))$.
	\end{theorem}
	
	As before, let $k = |\opt|$. Let $U^{(t)}$ be the elements remaining at the start of round $t$, let $S^{(t)}$ be the set selected in round $t$, let $v^{(t)}$ be the element that arrives in round $t$, and let $x^{(t)}$ be the distribution $x$ at the start of round $t$. For convenience, we also define $ x_v^{(t)} := \sum_{S \ni v} x^{(t)}_{S}$.
	
	Define a potential $\Phi(t) = 2k\cdot \KL{x^*}{x^{(t)}} + 2(e-1)k \cdot\log \ \lvert U^{(t)} \rvert$, where $x^*$ is the uniform distribution on $\opt$. 
	Note that $\KL{x^*}{x^{(0)}} = \frac{1}{k} \sum_{S \in \opt} \log (m/k) = \log (m/k)$, and $\log |U^{(0)}| = \log n$, and hence $\Phi(0) = k \cdot \log (mn/k)$.
	
	We bound the expected decrease in each term of this potential separately.
	
	\begin{claim}
	\label{lem:polytime_klchange}
	    The expected change in relative entropy is
		\[\expectover{\substack{v \sim U^{(t)} \\ S \sim x^{(t)}}}*{ \KL{x^*}{x^{(t+1)}} - \KL{x^*}{x^{(t)}} \mid x^{(t)}, U^{(t)}} \leq \expectover{v \sim U^{(t)}}*{x^{(t)}_v} - \frac{1}{k}.\]
	\end{claim}
	\begin{proof}
	The change in relative entropy only depends on $v^{(t)}$, not $S^{(t)}$. Hence
	\begin{align*}
	        & \expectover{\substack{v \sim U^{(t)} \\ S \sim x^{(t)}}}*{\KL{x^*}{x^{(t+1)}} - \KL{x^*}{x^{(t)}} \mid x^{(t)}, U^{(t)}} \\
	        &= \expectover{v \sim U^{(t)}}*{\sum_{S} x^*_S \log \frac{x^{(t)}_S}{x^{(t+1)}_S}} \\
     	        &= \expectover{v \sim U^{(t)}}*{\sum_{S} x^*_S \cdot  \log Z^{(t)} - \sum_{S \ni v} x^*_S }. \\
     	        \intertext{Since $\opt$ is a feasible cover and $x^*$ is the uniform distribution on $\opt$,}
	        &= \expectover{v \sim U^{(t)}}*{\sum_{S \ni v} x^*_S \log (1+ (e-1) \cdot x^{(t)}_{e})} - \frac{1}{k} \\
	        &\leq \expectover{v \sim U^{(t)}}*{\log(1+(e-1) \cdot x^{(t)}_v)} - \frac{1}{k}. \\
	        \intertext{Using the approximation $\log (1+x) \leq x$, this is}
	        &\leq (e-1)\cdot \expectover{v \sim U^{(t)}}*{x^{(t)}_v} - \frac{1}{k}. \qedhere
	    \end{align*}
	\end{proof}
	
	\begin{claim}
	\label{lem:polytime_utchange}
	    If $|U^{(t+1)}| \geq 1$ then the expected change in $\log \ \lvert U^{(t)} \rvert$ is
		\[\expectover{\substack{v \sim U^{(t)} \\ S \sim x^{(t)}}}*{\log \  \lvert U^{(t+1)}\rvert - \log \ \lvert U^{(t)}\rvert | x^{(t)}, U^{(t)}} \leq - \expectover{v \sim U^{(t)}}*{x^{(t)}_v}. \]
	\end{claim}
	\begin{proof}
	The change in $\log \ \lvert U^{(t)} \rvert$ only depends on $S^{(t)}$, not $v^{(t)}$. Hence
	\begin{align*}
	        &\expectover{S \sim x^{(t)}}*{\log \ \lvert U^{(t+1)} \rvert - \log \ \lvert U^{(t)} \rvert \ | x^{(t)}, U^{(t)}} \\
	        &= \expectover{S \sim x^{(t)}}*{\log \left(1-\frac{\lvert S \rvert}{\lvert U^{(t)} \rvert} \right)} \\
	        &\leq - \expectover{S \sim x^{(t)}}*{\frac{\lvert S \rvert}{\lvert U^{(t)} \rvert} } \\
	        &= -\frac{1}{\lvert U^{(t)} \rvert} \sum_S \sum_{u \in S} x^{(t)}_S \\
	        &= -\frac{1}{\lvert U^{(t)} \rvert} \sum_{u} x^{(t)}_u \\
	        &= -\expectover{v \sim U^{(t)}}*{x^{(t)}_v}. \qedhere
	    \end{align*}
	\end{proof}
	
	\begin{proof}[Proof of \cref{thm:unit_cost_poly}]
	Combining claims \cref{lem:polytime_klchange} and
        \cref{lem:polytime_utchange}, we have
        \begin{align*}
        	&\expectover{\substack{v \sim U^{(t)} \\ \mathcal{R} \sim x^{(t)}}}*{\Phi(t) - \Phi(t-1) | e^{(1)}, \ldots, e^{(t-1)}, \mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(t-1)}} \\
        & = \expectover{\substack{v \sim U^{(t)} \\ \mathcal{R} \sim x^{(t)}}}*{
        	\begin{array}{ll}
        		&2k\left(\KL{x^*}{x^{(t+1)}} - \KL{x^*}{x^{(t)}}\right) \\
        		+ &2k(e-1)\left(\log \ \lvert U^{(t+1)} \rvert - \log \ \lvert U^{(t)} \rvert\right)
        	\end{array}
        	 | e^{(1)}, \ldots, e^{(t-1)}, \mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(t-1)}} \\
         &= -2.
        \end{align*}
        In every round, the algorithm buys at most $2$ sets, which yields the inequality
	\[\expectover{\substack{v \sim U^{(t)} \\ \mathcal{R} \sim x^{(t)}}}*{\Phi(t) - \Phi(t-1) + c(\alg(t)) - c(\alg(t-1)) | e^{(1)}, \ldots, e^{(t-1)}, \mathcal{R}^{(1)}, \ldots, \mathcal{R}^{(t-1)}} \leq 0.\]
	The claim follows by applying \cref{lem:exp_pot_change} and
   by the bound on the starting potential, $\Phi(0) \leq k \cdot  \log
        (mn/k)$. 
	\qedhere
\end{proof}
	
